QueryBooster: Improving SQL Performance Using Middleware Services for Human-Centered Query Rewriting

SQL query performance is critical in database applications, and query rewriting is a technique that transforms an original query into an equivalent query with a better performance. In a wide range of database-supported systems, there is a unique problem where both the application and database layer are black boxes, and the developers need to use their knowledge about the data and domain to rewrite queries sent from the application to the database for better performance. Unfortunately, existing solutions do not give the users enough freedom to express their rewriting needs. To address this problem, we propose QueryBooster, a novel middleware-based service architecture for human-centered query rewriting, where users can use its expressive and easy-to-use rule language (called VarSQL) to formulate rewriting rules based on their needs. It also allows users to express rewriting intentions by providing examples of the original query and its rewritten query. QueryBooster automatically generalizes them to rewriting rules and suggests high-quality ones. We conduct a user study to show the benefits of VarSQL to formulate rewriting rules. Our experiments on real and synthetic workloads show the effectiveness of the rule-suggesting framework and the significant advantages of using QueryBooster for human-centered query rewriting to improve the end-to-end query performance.

==> backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - origianl table 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\footnotesize
\caption{Suitability of existing languages for \sysname.}
\label{tab:rule-langs}
\begin{tabular}{|l|ll|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Rule\\ Language\end{tabular}}} & \multicolumn{2}{l|}{\textbf{Expressive Power}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Indepen-\\dent of\\ DB\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}No Know-\\ledge be-\\sides SQL$^*$\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Additional \\ Knowledge \\ Users Need\end{tabular}}} \\ \cline{2-3}
 & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}SQL \\ Semantics\end{tabular}}} & \textit{\begin{tabular}[c]{@{}l@{}}SQL \\ Schema\end{tabular}} &  &  &  \\ \hline
\textbf{Regex} & \multicolumn{1}{l|}{No} & No & \textbf{Yes} & \textbf{Yes} &  \\ \hline
\textbf{Comby} & \multicolumn{1}{l|}{No} & No & \textbf{Yes} & \textbf{Yes} &  \\ \hline
\textbf{KOLA} & \multicolumn{1}{l|}{\textbf{Yes}} & No & \textbf{Yes} & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2} \circled{3}\end{tabular} \\ \hline
\textbf{EDS} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & No & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2}\end{tabular} \\ \hline
\textbf{Exodus} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & No & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2}\end{tabular} \\ \hline
\textbf{Starburst} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & No & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2} \circled{4} \circled{5}\end{tabular} \\ \hline
\textbf{Prairie} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & No & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2} \circled{5}\end{tabular} \\ \hline
\textbf{Calcite} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & \textbf{Yes} & No & \begin{tabular}[c]{@{}l@{}}\circled{1} \circled{2} \circled{4} \circled{6}\end{tabular} \\ \hline
\textbf{VarSQL} & \multicolumn{1}{l|}{\textbf{Yes}} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} &  \\ \hline
\end{tabular}
  \rfour{\footnotesize{$^*$ Excluding the syntax of the rule language itself since it is needed for any language.}}
  \circled{1} Query Optimization; \circled{2} Relational Algebra; \circled{3} Combinator-based Algebra; 
  \\
  \circled{4} Internal Data Structure; \circled{5} C++ Programming; \circled{6} Java Programming;
\vspace{-2pt}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SQL query performance is critical in database applications, and query rewriting is an optimization technique that can transform an original query to an equivalent query and improve its performance.  With the prevalent use of Business Intelligence applications and Object Relational Mapping frameworks for web development, existing databases and rewriting solutions miss many opportunities of rewriting the machine-generated SQL queries due to their non-intuitiveness and domain-specific inefficiency.  We propose \sysname, a middleware service for human-centered query rewriting, where users can leverage their domain knowledge to introduce data and application-specific rewriting rules to improve the query performance.  \sysname provides an expressive and easy-to-use rule language (called \langname) for users to formulate rewriting rules. It also allows users to express their rewriting intentions by providing rewriting examples of original queries and rewritten queries, and \sysname automatically generalizes them into rewriting rules and suggests high-quality ones to the users.  We conduct a user study to show the benefit of using the \langname rule language to formulate rewriting rules.  Our experiments on real and synthetic workloads show the effectiveness the rule-suggesting framework and the significant advantages of using \sysname for human-centered query rewriting to improve the end-to-end query performance.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boldstart{Performance is important.}  

\qiushi{
System performance is critical in many database applications where users need answers quickly to gain timely insights and make mission-critical decisions.
}

\boldstart{Query rewriting is one technique.}

\qiushi{
In the large body of optimization literature~\cite{conf/icde/FinanceG91, journals/vldb/KossmannPN22, conf/sigmod/PiraheshHH92}, one family of technique is ``query rewriting,'' which transforms an original query to a semantically equivalent alternative query that can be evaluated by the database engine more efficiently.
}

\boldstart{Despite the success of automatic query rewriting, we still need ``human-centered'' query rewriting.}

\qiushi{
Automatic query rewriting~\cite{journals/debu/Graefe95a, journals/tkde/Graefe94} inside databases has been studied extensively in the literature, including adding hints~\cite{conf/sigmod/MarcusNMTAK21, journals/corr/abs-2112-00182, journals/pvldb/DamasioCGMMSZ19}, re-ordering rewriting rules~\cite{journals/pvldb/ZhouLCF21}, and discovering new rules~\cite{conf/sigmod/WangZYDHDT0022}.  However, it is insufficient to rely on existing rewriting solutions for queries generated from BI (Business Intelligence) systems such as Tableau and web applications developed using ORM (Object Relational Mapping) frameworks.  Different than human-crafted queries, these machine-generated queries can be non-intuitive for databases to optimize~\cite{conf/sigmod/WangZYDHDT0022}, or use in-efficient expressions for computations (as shown in Section~\ref{sec:need-for-human-centered-query-rewriting}), which require humans to rewrite them into more efficient forms.  In those cases, SQL developers need to leverage their domain knowledge to introduce data or application-specific rewriting rules to rewrite their queries and improve the query performance.  We call this ``human-centered query rewiring''.  Our experiments (Section~\ref{sec:end-to-end-query-time}) show that among the $20$ TPC-H queries formulated by Tableau on top of Postgres, $50\%$ can be further optimized by human-crafted rewriting rules and accelerated by up to $86\%$.
}

\boldstart{Unfortunately, existing solutions cannot satisfy this need.}  

\qiushi{
Unfortunately, despite the great need of human-centered query rewriting within the life-cycle of the query optimization, existing databases and third-party rewriting tools can barely satisfy this need.  In our study (details in Section~\ref{sec:lack-of-support-in-existing-solutions}), most commercial databases don't have a user interface for developers to define their own rewriting rules except Postgres and MySQL, while the interfaces of both the latter systems are too limited for users to express their desired rewriting rules.  Third-party solutions mainly focus on automatic query rewriting with existing rules or discovering new rules without human-involvement, and none of them offers an interface for users to express their own rewriting needs.
}

\boldstart{Our solution.}

\qiushi{
In this paper, we propose \sysname, a middleware service for human-centered query rewriting.  It sits in between the application and database to intercept SQL queries sent from the application and rewrite them using human-crafted rewriting rules to improve the queries' performance.  By providing a slightly-modified JDBC/ODBC driver or a RESTful proxy for the query interception, \sysname requires \textbf{{\em zero}} code changes to either the application or the database.  \sysname provides a powerful interface for users to formulate rewriting rules in two ways.  First, it provides an expressive and easy-to-use rule language (called \langname) for users to define rewriting rules.  Uses can easily express their rewriting needs by writing down the query pattern and its replacement.  They can also specify additional constraints and actions for complex rewriting details.  Second, it allows users to express their rewriting intentions by providing examples.  Users can input original queries and the desired rewritten queries and \sysname automatically generalizes the examples into rewriting rules and suggests high-quality rules to the users.  The users can confirm the rules to be persisted into the system or further modify the rules as they want.  
}

\boldstart{Challenges.}

\qiushi{
To develop the \sysname system, we faced a few challenges. \textbf{(C1)} How to develop an expressive and easy-to-use rule language for users to formulate rules?  \textbf{(C2)} How to generalize pairs of original and rewritten queries to rewriting rules and measure their qualities?  and \textbf{(C3)} How to search the candidate rewriting rules to suggest high-quality ones based on the user-given examples?  To address these challenges, our work makes the following contributions:
}

\boldstart{Our contributions.}

\qiushi{
\begin{itemize}
    \item We propose a novel middleware-based query rewriting service to fulfill the urgent need of human-centered query rewriting (Section~\ref{sec:querybooster-middleware}).
    \item We study the suitability of existing rule languages in the literature and develop a novel rule language (\langname) that is expressive and easy to use (Section~\ref{sec:rule-lang}).
    \item We design a few transformations to generalize pairs of rewriting queries to rewriting rules and propose using the Minimum Description Length metric to measure rule qualities (Section~\ref{sec:rule-qualities-and-transformations}).
    \item We develop a greedy-search framework to search the candidate rewriting rules efficiently and suggest high-quality rewriting rules based on user-given examples (Section~\ref{sec:searching-high-quality-rules}).
    \item We conduct a user study and thorough experiments to show the benefit of the \langname rule language, the effectiveness of the rule-suggesting framework, and the advantages of human-centered query rewriting. (Section~\ref{sec:experiments})
\end{itemize}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - sec 2 motivation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Motivation}

In this section, we show the need for human-centered query rewriting between applications and databases, and the lack of support in existing database solutions.

\subsection{Need for Human-Centered Query Rewriting \label{sec:need-for-human-centered-query-rewriting}}

\begin{wrapfigure}{r}{0.4\linewidth}
 \centering
    \includegraphics[scale=.75]{figures/tableau-on-postgres}
    \caption{Query lifecycle of Tableau on Postgres.}
  \label{fig:tableau-on-postgres}
\end{wrapfigure}

System performance is critical in many database applications where users need answers quickly to gain timely insights and make mission-critical decisions.  In the large body of optimization literature~\cite{conf/icde/FinanceG91, journals/vldb/KossmannPN22, conf/sigmod/PiraheshHH92}, one family of technique is ``query rewriting,'' which transforms a query $Q$ to a new query $Q'$ such that $Q'$ computes the same answers as $Q$, but runs much faster. For example, Figure~\ref{fig:tableau-on-postgres} shows a case where a user runs Tableau on top of a Postgres database to analyze and visualize the underlying data of social media tweets.  Tableau formulates and sends a SQL query to the database for each frontend request through a connector such as a JDBC driver.  The database returns the result to Tableau to render in the frontend.

Figure~\ref{fig:original-query-strpos} shows an example SQL query $Q$ formulated by Tableau to compute a choropleth map of tweets containing a substring, e.g., {\tt covid}, which matches {\tt covid-19}, {\tt covid19}, {\tt postcovid}, {\tt covidvaccine}, etc.  Without any index available on the table, the database engine uses a scan-based physical plan that takes $34$ seconds.  The developer is tempted to create an index on the \texttt{content} attribute of the table to improve the performance.

\begin{figure}[htbp]
  \centering
  \begin{subfigure}[t]{0.48\linewidth}
    \begin{sqlnotitle}
SELECT SUM(1) AS "cnt:tweets",
                    "state_name" AS "state_name"
FROM "tweets"
WHERE &STRPOS(LOWER("content"),
                    'covid') > 0& 
GROUP BY 2;
    \end{sqlnotitle}
    \caption{An original query $Q$ formulated by Tableau to compute a choropleth map of tweets containing {\tt covid} substring. \label{fig:original-query-strpos}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\linewidth}
    \begin{sqlnotitle}
SELECT SUM(1) AS "cnt:tweets",
                    "state_name" AS "state_name"
FROM "tweets"
WHERE &"content" ILIKE 
                    '%covid%'&
GROUP BY 2;
    \end{sqlnotitle}
    \caption{A rewritten query $Q'$ equivalent to $Q$ but runs 100 times faster by using a trigram index on {\tt content}. \label{fig:rewritten-query-strpos}}
  \end{subfigure}
  \caption{An example query pair (differences shown in blue).}
  \label{fig:rewrite-example-strpos}
\end{figure}

Unfortunately, Postgres does not support an index-based physical plan for the \texttt{STRPOS(LOWER("content"),$s$)} expression in $Q$, where $s$ is an arbitrary string. Interestingly, another query $Q'$, shown in Figure~\ref{fig:rewritten-query-strpos}, is equivalent to $Q$, and uses an \texttt{ILIKE} predicate.  This expression can be answered using a trigram index on the \texttt{content} attribute~\cite{postgres:trigram}, and the corresponding physical plan takes $0.32$ seconds only.  Notice that the optimizer does not produce an index-based plan for the original {\tt STRPOS} predicate using this trigram index~\cite{email:index-in-strpos-function}.

A natural question is whether we can let Tableau generate $Q'$ instead of $Q$ for the database.  Unfortunately, Tableau is a proprietary application layer with its own internal logic to generate queries, which the developer, in this example, cannot change.  Furthermore, for legacy systems~\cite{conf/sigmod/KhuranaH21}, the source code may be too old and complicated to modify or even unavailable to developers.  For example, reports~\cite{blog:software-is-fragile} show many applications where parties have lost their source code.

To this end, developers need to leverage their knowledge about the data and domain to rewrite queries sent from the application to the database to improve their performance significantly.  For example, they may introduce rewriting rules that are valid for their particular database with certain properties (e.g., specific attribute types, certain cardinality constraints, or primary keys and foreign keys), even though these rules may not be valid for all databases.  We call this idea of putting developers ``in the driver's seat'' during the lifecycle of a query to generate an equivalent yet significantly more efficient query as ``human-centered query rewiring''.  Next, we show the lack of support for human-centered query rewriting in native and third-party database solutions.

\subsection{Lack of Support in Existing Solutions \label{sec:lack-of-support-in-existing-solutions}}

Figure~\ref{fig:query-rewriting-systems} gives an overview of existing solutions for query rewriting in the lifecycle of a query in a database system~\cite{calcite, journals/pvldb/DamasioCGMMSZ19, conf/sigmod/MarcusNMTAK21, conf/sigmod/WangZYDHDT0022, journals/pvldb/ZhouLCF21} and the position of the proposed \sysname system.  At a high level, these solutions can be classified into two categories: native writing plugins and third-party solutions.

\begin{figure}[htb]
  \centering
  \includegraphics[width=.99\linewidth]{figures/query-rewriting-systems}
  \caption{Query-rewriting solutions for databases (native in brown, third-party in blue).}
  \label{fig:query-rewriting-systems}
\end{figure}

\boldstart{Native rewriting plugins.}  Most databases such as AsterixDB~\cite{asterix:website}, IBM DB2~\cite{db2:doc}, MongoDB~\cite{mongodb:doc}, MS SQL Server~\cite{sqlserver:doc}, MySQL~\cite{mysql:query-rewrite}, Oracle~\cite{oracle:query-rewrite}, Postgres~\cite{postgres:query-rewrite}, SAP HANA~\cite{hana:doc},  Snowflake~\cite{snowflake:website}, and Teradata~\cite{teradata:website}, do not have capabilities for users to rewrite queries sent to the database.  Notice that even though ``hints'' can be included in a query to make suggestions to the database optimizer, technically, they are not used to change the query, thus, are not a query-rewriting solution.  Only two database systems, Postgres and MySQL, provide a plugin for users to define new rules to rewrite queries before sending them to the database.  However, their rule-definition languages have limited expressive power, as discussed below.  

\boldstart{Postgres.} A rewriting rule in the Postgres plugin can only define a pattern matching a table name in a {\sf SELECT} clause of a SQL query and replace the table with another table or a subquery~\cite{postgres:query-rewrite}.  Its rule language cannot express the rewriting in the running example in Figure~\ref{fig:rewrite-example-strpos}.  In particular, it does not support a pattern that matches a component in a SQL statement at the predicate level, e.g., the \texttt{STRPOS(LOWER("content"), \_) > 0} portion in the {\tt WHERE} clause in the original query.  Safety could be a major consideration behind this rule language.  For instance, the Postgres 14 documentation~\cite{postgres14:doc} explained that ``{\em this restriction was required to make rules safe enough to open them for ordinary users, and it restricts ON SELECT rules to act like views}.''

\boldstart{MySQL.}  The MySQL plugin uses the syntax of prepared statements to define query-rewriting rules, and a rule replaces a SQL query matching the rule's pattern with a new statement~\cite{mysql:query-rewrite}.  A rule includes placeholders that can only match literal values in a SQL query, such as a constant in a predicate in the {\tt WHERE} clause. A main limitation of this language is that a placeholder cannot match many components in a query, such as table names, attribute names, function names (e.g., {\tt CAST}), and SQL reserved words (e.g., {\tt DATE}).   For instance, the following is a predicate from a query formulated by Tableau to MySQL:

\begin{rule-example}
adddate(date_format(`created_at`, '$\%$Y-$\%$m-$01$ $00$:$00$:$00$'), 
                   interval $0$ second) = TIMESTAMP('$2018$-$04$-$01$ $00$:$00$:$00$')
\end{rule-example}

MySQL allows the creation of an index on the derived column of the left-hand operand of the predicate.  However, the query cannot use the index due to the data type mismatch between the left-hand and right-hand operands in the predicate~\cite{blog:mysql-not-using-index}.  In particular, the data type of the left-hand expression is \texttt{string} because the \texttt{adddate} function maintains the data type of the first argument~\cite{mysql:adddate} (i.e., \texttt{date\_format('created\_at', '\%Y-\%m-01 00:00:00')}), which is a \texttt{string}.  The right-hand operand is a \texttt{Timestamp} type.  To solve the problem, we can rewrite the predicate by removing the type-casting on the right-hand constant, as shown below:

\begin{rule-example}
adddate(date_format('created_at', '$\%$Y-$\%$m-$01$ $00$:$00$:$00$'), 
                   interval $0$ second) = '$2018$-$04$-$01$ $00$:$00$:$00$'
\end{rule-example}
The corresponding rewritten query is significantly faster ($2.68$s) than the original query ($87$s).  Unfortunately, the MySQL plugin does not support this rewriting because a pattern in the MySQL plugin has to be an {\em entire} statement instead of a {\em single} predicate.

\boldstart{Third-party solutions.}  Bao~\cite{conf/sigmod/MarcusNMTAK21} and Galo~\cite{journals/pvldb/DamasioCGMMSZ19} rewrite queries by adding hints to help the database optimizer generate more efficient physical plans based on their cost estimations and searching methods.  They take a physical plan and query performance as the input and produce hints to the original query.  WeTune~\cite{conf/sigmod/WangZYDHDT0022} generates new rewriting rules automatically by searching the logical-plan space and considering the performance of rewritten queries.  LearnedRewrite~\cite{journals/pvldb/ZhouLCF21} utilizes built-in rewriting rules inside the database to optimize queries, and the users have no control over when and which rules are applied. 
None of these solutions allow users to formulate their own rewriting rules to fulfill the human-centered query rewriting need.

%\boldstart{Uniqueness of \sysname.}  To our best knowledge, the proposed system is the only solution that allows users to define their own rules to rewrite queries before the queries are sent to the database.  In this way, it can not only provide a chance for the users to add rules based on their domain knowledge but also allow minimal or no changes to the application and database. 

% \boldstart{Other related work.} There are also commercial systems that do query rewriting for applications on top of databases.  For example, Keebo~\cite{keebo:website} uses data learning and {\em approximate} query processing (AQP) techniques to accelerate analytical queries between applications and databases.  It runs queries on summarized tables instead of the raw data as much as possible to reduce query time.  EverSQL~\cite{eversql:website} uses AI/ML techniques to recommend rewriting ideas for queries on MySQL and Postgres.  Other systems such as ApexSQL~\cite{apexsql:website}, Query Performance Insights for Azure SQL~\cite{query-insight-azure-sql:website}, and Toad~\cite{toad:website} help database developers analyze query performance bottlenecks and tune database knobs.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - advantages of imperative languages against declarative languages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main advantage of imperative languages is the expressive power offered by the programming language (e.g., Java), such as defining schema-dependent pattern-matching conditions.  Consider the example query pair based on the Q18 query in the TPC-H benchmark~\cite{TPC-H} shown in Figure~\ref{fig:tableau-plus-tpc-h-workload}.  We want to rewrite the join predicate on the derived table \texttt{t1} and raw table \texttt{orders} from the original ``\texttt{IS NOT DISTINCT FROM}'' (in blue) to an equality condition.  The predicate $$``\texttt{x IS NOT DISTINCT FROM y}''$$
is equivalent to 
$$``\texttt{(x is NULL and y is NULL) OR x = y}'',$$ which joins two rows if either the join columns have the same non-NULL value or they are both \texttt{NULL}.  In our example, since the join column \texttt{l\_orderkey} is a primary key in table \texttt{orders} and a foreign key in table \texttt{lineitem} and it has no \texttt{NULL} values, we can safely convert the join condition to an equal join.   However, to check if we can do this transformation, we need schema information from the database, which cannot be inferred just from the SQL query itself.  Using an imperative rule engine, we can easily write a rule with a few lines of C code~\cite{conf/icde/PiraheskLH97} that accesses the schema data and checks the matching condition.  

\begin{figure}[tb]
  \centering
  \begin{subfigure}[t]{0.42\linewidth}
    \begin{sqlnotitle}
    SELECT customer.c_name,
                        SUM(t1.o_quantity)
      FROM (
    select l_orderkey, 
                  sum(l_quantity) as o_quantity
      from lineitem
     group by l_orderkey
     having sum(l_quantity) > = 301
  ) t1
  LEFT JOIN orders o ON 
      &(t1.l_orderkey IS NOT 
        DISTINCT FROM o.l_orderkey)&
  LEFT JOIN customer c ON 
      (orders.o_custkey = c.c_custkey)
 GROUP BY 1;
    \end{sqlnotitle}
    \caption{The original query ($Q$).}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.5\linewidth}
    \begin{sqlnotitle}
   SELECT customer.c_name,
                        SUM(t1.o_quantity)
      FROM (
    select l_orderkey, 
                  sum(l_quantity) as o_quantity
      from lineitem
     group by l_orderkey
     having sum(l_quantity) > = 301
  ) t1
  LEFT JOIN orders o ON 
      &(t1.l_orderkey = 
        o.o_orderkey)&
  LEFT JOIN customer c ON 
      (orders.o_custkey = c.c_custkey)
 GROUP BY 1;
    \end{sqlnotitle}
    \caption{The rewritten query ($Q'$).}
  \end{subfigure}
  \caption{An example query-rewriting pair in an application of Tableau and Postgres (differences shown in blue).}
  \label{fig:tableau-plus-tpc-h-workload}
\end{figure}

% One way to solve the problem is to provide a pre-defined imperative function to the declarative language.  For example, suppose we implement a procedure called \texttt{IS\_PFKEY(x)} that checks if the column \texttt{x} is a primary key or a foreign key in the table.  Then we can formulate a rule to rewrite the join predicate.  An example rule using the EDS language enhanced with our imperative procedure is shown below:

% \begin{rule-example}
% JOIN (t1, t2, t1.x IS NOT DISTINCT FROM t2.y) / 
% IS_PFKEY (x) | IS_PFKEY (y) --> JOIN (t1, t2, t1.x = t2.y).
% \end{rule-example}

% To this end, \sysname prefers a declarative rule language because it significantly ``lowers the bar'' without exposing the rule engine's details to users.  Additionally, it needs flexibility from the imperative languages, such as inferring types and keys from the database schema.  \qiushi{In summary, besides the three requirements shown above, \sysname has two more requirements for the rule language.  First, \textbf{(r4) it should be a declarative language.}  Second, \textbf{(r5) it should support the flexibility imperative languages provide.}}  With all the requirements in mind, we present a novel rule language called \langname.

% that combines the advantages of general and SQL-specific languages and declarative and imperative languages.  We present the details in the following subsection.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Syntax Diagram Example
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=.7\linewidth]{figures/result-column-diagram}
%     \caption{\qiushi{The syntax diagram of a ``result-column'' in the \texttt{SELECT} clause of a pattern query in \langname. Based on the original syntax diagram for SQLite, the difference is highlighted in blue color, where a variable is an alternative to an expression or a table name.}}
%     \label{fig:result-column-diagram}
% \end{figure}

% \qiushi{The syntax of \langname to formulate a pattern or replacement SQL query is the same as the original SQL syntax.  The only difference is that \langname introduces two types of variables as alternatives to the corresponding SQL elements.  Thus, we can formally define \langname's grammar using SQL syntax diagrams by adding those variables.  For example, Figure~\ref{fig:result-column-diagram} shows the syntax diagram of a ``result-column'' in the \texttt{SELECT} clause of a pattern query.  It is based on the original syntax diagram of a ``result-column'' for an SQLite query and the difference is the two places where a variable can be used.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Backup - Order Insensitive pattern matching in VarSQL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boldstart{SQL syntax tree-based pattern matching and replacing.}  \langname operates the pattern matching and replacing at the SQL syntax tree level, other than general languages such as Regex and Comby that operate at the string level or SQL-specific languages such as EDS and KOLA that operate at the query logical plan level.  On one hand, the major problem of operating at the string level is that the order of elements in the pattern is important.  For example, in Comby, if the pattern is defined as $$\texttt{SELECT * FROM orders, customers},$$ it does not match a query with a different order of joining the same two tables, such as $$\texttt{SELECT * FROM customers, orders}.$$  This is counter-intuitive for SQL users because, in SQL semantics, the above two queries share the same pattern.  On the other hand, operating at the query logical plan level solves the problem, but it requires users additional knowledge of translating a SQL query into a logical plan to use the language.  Thus, \langname operating at the SQL syntax tree level provides the order-insensitive pattern matching ability and requires no additional knowledge besides SQL.  We now explain the pattern matching and replacing process of \langname rule on an example query.  Consider the rule $R$ shown at the bottom of Figure~\ref{fig:rewrite-process} where the pattern and replacement are shown in their syntax tree formats.  This rule specifies that when two tables with the same name join on the same unique column, we can safely remove the join and keep only one copy of the table.  The remaining of Figure~\ref{fig:rewrite-process} shows the pattern matching and replacing process of this rule on an example query $Q$.  We first obtain the syntax tree of the query, and then compare it node by node against the syntax tree of rule's pattern.  The keyword nodes all match each other and the variables in the pattern match those elements in the query.  Under the node ``\texttt{and}'', the subtree ``\texttt{<t1>.<a1>=<t2>.<a2>}'' in the pattern matches the predicate ``\texttt{e1.id=e2.id}'' in the query and the set-variable ``\texttt{<<p>>}'' matches the two remaining predicates in the query.  Next, we use the rule's replacement syntax tree as a template to generate the rewritten query's syntax tree by replacing the variables with their matched elements in the pattern.  Finally, we assemble the rewritten query from the syntax tree.  For completeness, we also show the string representation of the rule $R$ in Figure~\ref{fig:rule-remove-self-join}.

%\boldstart{Order-insensitive pattern matching inside a clause.}  A problem of general rule languages such as \langname, Comby, and Regex, where a plain SQL string defines a rule pattern, is that the order of elements in the pattern is important.  For example, in Comby, if the pattern is defined as $$\texttt{SELECT * FROM orders, customers},$$ it does not match a query with a different order of joining the same two tables, such as $$\texttt{SELECT * FROM customers, orders}.$$  \qiushi{This is counter-intuitive for SQL users because, in SQL semantics, the above two queries share the same pattern.}  To solve this problem, \langname adopts the property of order-insensitive pattern matching widely used in SQL-specific languages.
%When a pattern matches a SQL query, \langname does not enforce the ordering of elements under a specific clause.  Consider a rule shown in Figure~\ref{fig:rule-remove-self-join}.  This rule specifies that when two tables with the same name join on the same unique column, we can safely remove the join and keep only one copy of the table.  This rule's pattern can match both queries shown in Figure~\ref{fig:examples-remove-self-join}, in which the join predicate (i.e., ``\texttt{<t1>.<a1>=<t2>.<a2>}'') and the predicate set-variable (i.e., ``\texttt{<{}<p>{}>}'') have different orders. This is also consistent with the order-insensitive nature of SQL queries, where different orders of the same set of predicates under a \texttt{WHERE} clause should yield the same result.

% \begin{figure}[tb]
%   \centering
%   \begin{subfigure}[t]{0.42\linewidth}
%     \begin{sqlnotitle}
%     SELECT e1.name, e1.age, e2.salary
%        FROM employee e1,
%                        employee e2
%      WHERE e1.id = e2.id
%             AND e1.age > 17
%             AND e2.salary > 35000;
%     \end{sqlnotitle}
%     \caption{An original query ($Q1$).}
%     \label{fig:q1-remove-self-join}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[t]{0.5\linewidth}
%     \begin{sqlnotitle}
%    SELECT sum(o1.total_price)
%        FROM orders o1,
%                        orders o2
%      WHERE o1.os in ('ios', 'macos')
%              AND o1.oid = o2.oid
%              AND o2.state_code = 'CA';
%     \end{sqlnotitle}
%     \caption{An original query ($Q2$).}
%     \label{fig:q2-remove-self-join}
%   \end{subfigure}
%   \caption{Two original queries that both can match the pattern of the rule in Figure~\ref{fig:rule-remove-self-join}.}
%   \label{fig:examples-remove-self-join}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> overflow.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Section 3.2 Need of a Powerful Rule Language
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Need of a Powerful Rule Language}

The main task of \sysname is to provide an expressive and easy-to-use interface for users to define rewriting rules that work for different applications and databases.  \sysname desires a rule language meeting requirements in three aspects, namely, expressiveness, convenience, and generality.

\boldstart{(R1) Powerful expressiveness in SQL semantics.}  To fulfill various and complex rewriting needs of users, \sysname requires the rule language to be powerful in expressing SQL semantics for rules.  It needs to allow users to specify pattern-matching conditions on the elements of a SQL query, e.g., two tables have the same name. It also allows the specification of rules on verifying conditions on the SQL schema, e.g., a column is unique in the table schema.  The expressiveness of the rule language should be powerful in that it understands SQL-specific semantics and supports schema-dependent pattern-matching conditions. 

\boldstart{(R2) Easy to use by SQL developers.}  Users of \sysname are application developers who are familiar with SQL. \sysname should require users to have little prior knowledge other than SQL to define their rewriting rules.  For example, a user should not need to know how the rewriting engine inside \sysname transforms SQL queries or how the execution engine inside the database computes the result of the SQL queries. 

\boldstart{(R3) Independent of databases or SQL dialects.}  \sysname is a general query-rewriting service that supports different applications and backend databases.  Its rule language should be independent of any specific database or SQL dialect.  For example, the syntax of defining a rewriting rule should not rely on a feature specific to a certain database or SQL dialect.

Providing a rule language that meets the aforementioned three requirements is challenging.  In Section~\ref{sec:rule-lang}  we first study the suitability of existing rule languages in the literature and then develop a novel rule language that combines advantages from existing languages to meet all the requirements. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Section 3.3 Suggesting Rules from User-Given Examples
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Suggesting Rules from User-Given Examples}

To make \sysname easy to use, it is important for users to be able to formulate high-quality rewriting rules with little effort.  Manually formulating a rewriting rule that covers many queries is tedious.  We want a better experience in which a user expresses the rewriting intention by providing query rewriting pairs.  Then, the system can automatically suggest rewriting rules to achieve the rewritings of the given examples.  For instance, if a user inputs the rewriting pair in Figure~\ref{fig:rewrite-example-strpos} as one of the examples, the rule suggestor can automatically generalize it and recommend the following rule to the user.

\begin{rule-example}
STRPOS(LOWER(<x>), '<y>') --> <x> ILIKE '%<y>%'
\end{rule-example}

The rule suggestor generalizes the examples into rewriting rules and suggests high-quality rules to the user.  
%The user can select the rewriting rules. The user can modify the suggested rules before saving them to the system.  
The user has full control of how the suggested rules are added to the rule base by selecting the rewriting rules to save or modifying the suggested rules as needed.
Upon seeing the output from the rule suggestor, the user may understand the rule language better and modify the input examples to express the rewriting intentions more accurately, and the rule suggestor can refine the suggestions based on the new examples.

Developing such a rule suggestor is also challenging since we need to answer a few questions, such as how to measure the quality of rewriting rules, how to generalize query rewriting pairs into rewriting rules, and how to search the candidate rewriting rules to suggest high-quality ones.  We answer these questions in Section~\ref{sec:rule-qualities-and-transformations} and Section~\ref{sec:searching-high-quality-rules}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Section 4.3 VarSQL-based Rewriting Engine
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\langname-based Rewriting Engine}

We briefly discuss how the rewriting engine is implemented in \sysname.  All user-formulated rules are stored in the rule base as shown in Figure~\ref{fig:architecture}.  When an original query $Q$ comes, the query rewriter accesses each rule $r$ in the rule base and checks its pattern and constraints against query $Q$.  If the rule $r$ matches $Q$, the query rewriter rewrites $Q$ to $Q'$ according to the rule's replacement and actions.  It then treats $Q'$ as $Q$ and repeats the rule matching and rewriting process until the query cannot match any rule in the rule base.  Note that the same rule can be matched and used multiple times.  

\boldstart{Termination of the rewriting process and the uniqueness of the result.}
To ensure the process always terminates, the query rewriter tracks the rewriting path and discovers cycles by checking if the same rewritten query appears more than once on the path.  It breaks a cycle by returning the repeated rewritten query as the result.  One concern is that different orders of applying rules on a query may result in different rewritten queries.  To address this concern, \sysname allows users to specify a priority for each rule so that high-priority rules can be applied first.  For example, a user may ask the system to apply general optimization rules (e.g., removing unnecessary type-castings) before applying specific optimization rules (e.g., replacing substring functions). To give users the full power to control the rewriting process, \sysname also provides a rule-management framework where a user can bundle a set of rules as a workspace and assign a specific database to the workspace so that the queries on the database will be rewritten only using the rules in the assigned workspace.

\boldstart{Supporting different databases and SQL dialects.}  \sysname can support different databases and SQL dialects for two reasons.  One is its simple design of extending SQL with variables.  The other is that the query rewriter operates at the Abstract Syntax Tree (AST) level and adopts existing SQL parsers to parse the queries and rules.  Existing rules are parsed into ASTs and then stored in the rule base.  For an input query, the query rewriter first parses the query into an AST.  It then does the pattern matching by comparing each rule's AST with the query's AST.  Once a rule pattern matches the query, the query rewriter assembles the rewritten query's AST based on the replacement AST of the rule.  Finally, it uses the same SQL parser to assemble the rewritten query's AST back to a SQL query.

Thus, \sysname can be easily extended to support different databases with different SQL dialects.  To support a new database and its SQL dialect, we replace the SQL parser inside the query rewriter with the corresponding SQL parser for the new database, and both the rule language and the query rewriting process can be adapted automatically. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Section 6.1 A Greedy Searching Framework (last paragraph)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This method has two problems.  One is that it is hard to decide the $k$ value.  A $k$ value may be good for some input examples but can be bad for others.  Figure~\ref{fig:k-hop-neighbors} shows an example where no transformed rules in the $1$-hop neighbors can reduce the total length of rules, thus it results in a local optimum. But searching for $2$-hop neighbors can find a globally optimal result.  The second problem is that a fixed $k$ value for all base rules ignores their different amounts of potential to discover a high-quality rule.  To solve these two problems, we propose an adaptive exploration method next.

\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{figures/k-hop-neighbors}
  \caption{An example of using the $k$-hop-neighbor method to explore candidates in Algorithm~\ref{alg:greedy}.  If $k=1$, the algorithm stops at the first iteration and returns the original pairs as the result with a total length of $20$.  If $k=2$, the algorithm stops at the second iteration and returns the $L7$ rule as the result with a total length of $12$.}
  \label{fig:k-hop-neighbors}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Section 6.2 Exploring Candidate Rules Adaptively
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% First figure
\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{figures/adaptive-exploration}
  \caption{The method of adaptive candidate exploration considers more promising transformed rules as the candidate rule set.}
  \label{fig:adaptive-exploration}
  \vspace{-2pt}
\end{figure}

%% Last paragraph
As an example, consider the candidate rule $c1$ in Figure~\ref{fig:distance-example}.  We want to compute the number of transformations $c1$ to cover the base rule $R_1$.  We first use $c_1$'s pattern to match $R_1$'s pattern and find those colored boxes of subtrees as mismatching parts between $c_1$ and $R_1$.  We then count, for each part, the number of needed transformations on $c_1$ to generate a more general form that covers $R_1$.  For instance, to transform the subtree ``\texttt{CAST(msg AS TEXT)}'' in $c_1$ to match the corresponding subtree ``\texttt{<x>}'' in $R_1$,  we first apply \textit{Variablize-a-Leaf} transformation to get a new subtree ``\texttt{CAST(<y> AS TEXT)}'', and then apply \textit{Variablize-a-Subtree} transformation to get the subtree ``\texttt{<z>}''.  In this way, the total number of transformations on $c_1$ to cover $R_1$ is four.  Note that there are cases when even though a transformed form $c'$ of a candidate rule can match a base rule $R_i$, the replacement of $c'$ may not rewrite $R_i$'s pattern to its replacement.  In this case, we treat the number of transformations on $c$ to cover $R_i$ as infinity and the term $\frac{\mathcal{L}(r_i)}{\mathcal{D}(c, R_i)}$ in the promisingness score function would be zero.  It means the candidate rule $c$ has no chance to cover the base rule $R_i$ no matter what transformations are applied.

%% Last figure
\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{figures/distance-example}
  \caption{An example of computing the number of transformations on a candidate rule $c_1$ to cover a base rule $R_1$.  The colored boxes show the mismatching parts between $c_1$ and $R_1$'s patterns.  The edges show the needed transformations on $c_1$ to generate a more general form that covers $R_1$.}
  \label{fig:distance-example}
\end{figure}

